Dynamics and Contracts for an Agent with Misspecified Beliefs

We study a single-agent contracting environment where the agent has misspecified beliefs about the outcome distributions for each chosen action. First, we show that for a myopic Bayesian learning agent with only two possible actions, the empirical frequency of the chosen actions converges to a Berk-Nash equilibrium. However, through a constructed example, we illustrate that this convergence in action frequencies fails when the agent has three or more actions. Furthermore, with multiple actions, even computing an $\varepsilon$-Berk-Nash equilibrium requires at least quasi-polynomial time under the Exponential Time Hypothesis (ETH) for the PPAD-class. This finding poses a significant challenge to the existence of simple learning dynamics that converge in action frequencies. Motivated by this challenge, we focus on the contract design problems for an agent with misspecified beliefs and two possible actions. We show that the revenue-optimal contract, under a Berk-Nash equilibrium, can be computed in polynomial time. Perhaps surprisingly, we show that even a minor degree of misspecification can result in a significant reduction in optimal revenue.

==> content/budget.tex <==
\section{Efficient Allocation for Agents with Budgets}
\label{sec:budget}
The principal wants to allocate an indivisible item to $n$ agents to maximize the social welfare. 
Each agent has a private value $\val$ drawn independently from a commonly known distribution $\dist$. 
Moreover, all agent has a hard budget constraint $\budget$ for purchasing the item. 
That is, for any agent~$i$ with value $\val_i$, the utility of the agent for receiving the item with probability $\alloc$ while paying price~$\price$ is 
\begin{align*}
\util_i(\alloc,\price; \val_i) = 
\begin{cases}
\val_i\alloc-\price & \price\leq \budget\\
-\infty & \price > \budget.
\end{cases}
\end{align*}
Moreover, for any pair $i\neq i'$, 
agent $i$ believes that the budget of the agent $i'$ is $\hat{\budget}$. 
We say that the agents are correctly specified if $\hat{\budget} = \budget$
and they are misspecified otherwise. 
% We consider the case that all agents are misspecified,
% i.e., all agents believe that the budgets of the opponents are $\hat{\budget} < \budget$. 

\paragraph{Mechanisms and Solution Concepts}
We consider sealed bid auctions where each agent $i$ makes a bid $\bid_i$, 
and allocation and payments are determined according to $\alloc$ and $\price$.
We adopt the solution concept analogous to \citet{esponda2016berk} 
when agents are misspecified. 


\begin{definition}\label{def:eqm}
A strategy profile $\strategy$ is a \emph{misspecified equilibrium} strategy if there exists a distribution over bids $G_i$ for each agent $i$ such that  
\begin{itemize}
    \item $G_i$ is the distribution over $\strategy_i(\val_i)$ (over the randomness of the valuation $\val_i$) conditional on the event that $\prob[b_{-i}\sim G_{-i}]{\price_i(\strategy_i(\val_i), b_{-i}) > \hat{\budget}} = 0$;
    \item $\strategy_i$ is agent $i$'s best response given competing bid distribution $G_{-i}$.
\end{itemize}
\end{definition}

Intuitively, this solution concept suggests that each agent will believe that any component's bid that induces budget infeasible payment is irrational, 
and remove those bids from consideration. 


In this paper, we will focus on designing mechanisms that are incentive compatible for agents with misspecified beliefs. 

\paragraph{Results}
When the agents are correctly specified, \citet{maskin2000auctions} shows that the all-pay auction is the welfare optimal mechanism, 
and there exists distributions such that the second best is strictly smaller than the first best.
We show that when agents are misspecified and $\hat{\budget} > \budget$, 
the optimal attained welfare coincide with the case of correctly specified agents
and the first best may not be attainable.

\begin{theorem}
When $\hat{\budget} > \budget$, 
the all pay auction is optimal and attains the same social welfare as the correctly specified case. 
\end{theorem}
\begin{proof}
For any mechanism $\mech$ and any corresponding misspecified equilibrium strategy profile~$\strategy$, 
according to \cref{def:eqm}, 
each agent $i$ cannot make any bid that leads to payment higher than $\budget$
since he is best responding to the opponents' bids distribution $G_{-i}$. 
Since $\hat{\budget} > \budget$, 
the event that $\prob[b_{-i}\sim G_{-i}]{\price_i(\strategy_i(\val_i), b_{-i}) > \hat{\budget}} = 0$
is also satisfied for any realization of $\strategy_i(\val_i)$. 
Hence $G_i$ is exactly the distribution over $\strategy_i(\val_i)$
and the strategy profile~$\strategy$ forms a Nash equilibrium. 
Therefore, the expected social welfare of mechanism $\mech$ in the misspecified setting coincides with its performance in the correctly specified setting, 
and the optimal is attained by the all pay auction.
\end{proof}


However, if $\hat{\budget} < \budget$, we can show that the first best outcome is always attainable.
% In fact, we will show that any feasible allocation rule is implementable. 
\begin{theorem}
When $\hat{\budget} < \budget$, there is a payment rule $\price$ that implements the efficient allocation $\alloc$. 
\end{theorem}
\begin{proof}
Given efficient allocation rule $\alloc$, 
let 
\begin{align*}
\hat{\alloc}_i(\val_i) = \expect[\val_{-i}]{\alloc(\val_i,\val_{-i}) \given \val_j\leq \hat{\budget}, \forall j\neq i}
\end{align*}
be the expected allocation conditional on the event that all opponents' bids are at most the misspecified budget $\hat{\budget}$.
It is easy to verify that $\hat{\alloc}_i(\val_i) = 1$ for all $\val_i > \hat{\budget}$.
Let 
\begin{align*}
\hat{\price}_i(\val_i) =  \val_i\cdot \hat{\alloc}_i(\val_i) - \int_{0}^{\val_i} \alloc(z) \dd z
\end{align*}
be the payment function that incentivize the agent to truthfully report his value if he believes the interim allocation rule is $\hat{\alloc}$. 
Note that $\hat{\price}_i(\val_i) \leq \hat{\budget}$
for all $\val_i$.

Fix the payment rule $\price_i(\val_i) = \hat{\price}_i(\val_i)$
if $\val_i \leq \hat{\budget}$
and $\price_i(\val_i) = \budget$ with probability $\frac{\hat{\price}_i(\val_i)}{\budget}$
and~0 with probability $1-\frac{\hat{\price}_i(\val_i)}{\budget}$
if $\val_i > \hat{\budget}$.
Given allocation $\alloc$ and payment $\price$, 
truthful bidding is a misspecified equilibrium. 
In particular, each agent $i$ will believe that each opponent's bid distribution is drawn from $\dist$ conditional on the event that the value does not exceeds $\hat{\budget}$, 
and hence the expected allocation given his belief is exactly $\hat{\alloc}$. 
Therefore, truthful reporting is a best response as both $\price$ and $\hat{\price}$ have the same expected payment, 
and the realizations never exceed the true budget $\budget$.
\end{proof}

\textbf{Remark:} Note that the design of this new mechanism is important for maximizing social welfare. 
If we just use the all-pay auction, which is optimal for the correctly specified model, 
when $\hat{\budget}$ is small, all agents with high value would never make bids higher than $\hat{\budget}$, and hence the mechanism cannot distinguish those values, 
which is bad for social welfare. 

==> content/frequentist.tex <==
\section{Dynamics and Contracts for a Frequentist Agent}

==> content/prel_gpt.tex <==
\section{Background and Model[chatGPT]}

% This section introduces key concepts integral to the subsequent discussions. We present the fundamentals of contract design, and the dynamics between a learning agent and a principal within this framework. Our focus rests on mis-specified agents, those whose beliefs about the outcome distribution or actions of other agents in the mechanism design setting do not encompass the actual outcome. The Berk-Nash Equilibrium is used as a solution concept for these mis-specified agents. We employ the term "objective" to differentiate the correctly specified setting from the mis-specified one.

% \subsection{General Contract Design}
% We consider a general contract design model with both moral hazard and adverse selection. 
% The agent has a private type $\type\in\types$
% and can flexibly choose any action from a finite set $\actions$. 
% In this model, there is a payoff relevant state $\state\in\states$
% and a contractable signal $\signal\in\signals$, 
% where both $\states$ and $\signals$ are finite sets.
% Each action $\action\in\actions$ determines a distribution $\statedist_{\action}$ over states and signals $(\state,\signal)$.
% The value of an agent with type $\type$ for choosing action $\action\in\actions$ given state $\state$ 
% is $\val(\type,\state,\action)$,
% and the agent has a linear preference on payments. 

% \paragraph{Contracts}
% A contract rule $\transfer:\signals\to \reals$ is a mapping from contractable signals to payments. 
% The principal can commit to a menu of randomized contracts. 
% The timeline of the contract game is shown as follows. 
% \begin{enumerate}
% \item The principal commits to a menu $\menu$ of randomized contracts. 
% \item An agent with type $\type$ chooses a menu option $\option\in\menu$, 
% and a contract $\transfer$ is realized according to distribution $\option$. 
% \item The agent chooses an action $\action\in \actions$
% and $(\state,\signal)$ are realized according to distribution~$\statedist_{\action}$.
% \item The agent pays price $\transfer(\signal)$ to the principal, 
% and the expected utility of the agent is 
% \begin{align*}
% \expect[(\state,\signal)\sim\dist_{\action}]{\val(\type,\state,\action) + \transfer(\signal)}. 
% \end{align*}
% \end{enumerate}

% This model includes several classic models in the literature as special cases:
% \begin{itemize}
% \item \textbf{auctions:} In monopoly auction setting, there is a binary action set $\actions = \{0,1\}$, 
% where $1$ represents winning the item. 
% The payoff relevant state is degenerate and hence can be omitted in this setting. 
% The value of an agent with type $\type$ for choosing action $\action$ is $\val(\type,\action) = \type\cdot\action$. 

% In this model, the signal space is also binary with $\signals = \{0,1\}$. 
% There is no moral hazard and $\signal=\action$ for any $\action\in\actions$ with probability $1$. 
% That is, the principal can directly design payments as a function of the allocation. 
% The classic objective in this setting is to maximize the expected revenue from the agent. 

% \item \textbf{contracts:} In classic contract design models, the agent's utility does not depend on the state, 

% \end{itemize}




\subsection{Objective Contract Design}

Contract design involves a principal aiming to assign a task to an agent. The agent can choose from a set of actions, $\actions$, with each action $a \in \actions$ incurring a cost $c(a)$ to the agent and leading to a distribution $T_a \in \Delta(\Omega)$ over potential outcomes $\Omega$. We denote by $t_a(\omega)$ the probability that if the agent chooses action $a\in \actions$, the realized outcome is $\omega\in \Omega$. The principal attributes a value $v(\omega)$ to each outcome $\omega \in \Omega$.

Although the principal can observe the outcomes $\omega$, the agent's actions remain hidden. A contract is characterized by a payment function $p: \Omega \rightarrow \mathbb{R}_+$, determined by the observed outcome $\omega$. The principal's objective is to design a contract that incentivizes the agent towards actions favorable to the principal, represented as:

\begin{equation*}
\max_{p} \mathbb{E}_{\omega \sim T_a} [v(\omega) - p(\omega)].
\end{equation*}

Simultaneously, the agent strives to maximize their expected utility, the difference between the payment received and their action's cost:

\begin{equation*}
\max_{a \in \actions} \mathbb{E}_{\omega \sim T_a} [p(\omega) - c(a)],
\end{equation*}

Designing the payment function $p$ to align both parties' objectives amidst the unobservable nature of the agent's actions poses a challenge for the principal. In simpler terms, the principal wants to maximize their expected net gain (value minus payment) for each outcome, while the agent seeks to maximize their expected utility (payment minus cost of action).

\subsection{Contract Design for a Learning Agent}\label{sec:learning agent}

We look into a scenario where an agent agrees to a \emph{static} contract $p$.\footnote{By static contract, we mean that the principal fixes the contract $p$.} The agent knows the cost function $c: \actions \rightarrow \mathbb{R}+$ that's related to her actions, but she's uncertain about the exact distribution of outcomes caused by her actions. To deal with this uncertainty, she has a set of beliefs $\Theta$. Each belief $\theta\in \Theta$ represents a distribution over outcomes $\theta_{a}\in \Delta(\Omega)$ for each possible action $a\in \actions$. She also has a prior belief $b_0 \in \Delta(\Theta)$ that reflects her initial assumptions about the action distribution.

At time $t$, the agent chooses an action $a_t \in \actions$ that maximizes her expected benefit, based on her updated belief $b_{t-1}$ from past experiences:
\begin{equation}
a_t=\argmax_{a \in \actions} \mathbb{E}_{\omega \sim b_{t-1}} [p(\omega) - c(a)].\label{eq:bayes action}
\end{equation}

After seeing the outcome $\omega_t$ from her action $a_t$, the agent updates her belief over distributions $\theta\in \Theta$ using Bayes' rule and the history of what she's seen so far $(a_1,\omega_1,\ldots,a_t,\omega_t)$:
\begin{equation}
b_{t}(\theta) \propto b_0(\theta)\cdot \prod_{t'\in[1,t]}\theta_{a_{t'}}(\omega_{t'}). \label{eq:bayes update}
\end{equation}


\subsection{Berk-Nash Equilibrium}

The Berk-Nash equilibrium, a concept stemming from Game Theory, is crucial when analyzing strategic interactions between players. When these players or agents have misconceptions or misunderstand the game's variables, we delve into a concept known as the misspecified Berk-Nash equilibrium.

In the context of a single-agent contract design, the Berk-Nash equiblirium is instantiated as following. Given a contract $p:\Omega\rightarrow\mathbb{R}_+$, suppose $\sigma^*\in \Delta(\actions)$ is a distribution over the agent's actions, and $\mu^*\in \Delta(\Theta)$ is a distribution over beliefs that form a Berk-Nash equilibrium. These distributions satisfy the following:

\begin{itemize}
    \item [Optimality:] For any action $a^*\in \text{supp}(\sigma^*)$ chosen by the agent, it must maximize her expected utility given her belief $\mu^*$:
    \begin{equation*}
        a^*\in \arg\max_{a\in A}\mathbb{E}_{\omega \sim \mu^*}[p(\omega)- c(a)]
    \end{equation*}
    Here, given a distribution over beliefs $\mu^*\in \Delta(\Theta)$, we also denote the distribution over outcomes as $\mu^*$.
    
    \item [Consistency:] Each belief $\theta^*\in \text{supp}(\mu^*)$ in the support of $\mu^*$ should minimize the following weighted Kullback-Leibler divergence from the true distribution of outcomes, given the agent's actions:
    \begin{equation*}
        \theta^*=\arg\min_{\theta\in \Theta}\sum_{a\in \text{supp}(\sigma^*)}\mathbb{E}_{\omega \sim T_a}\log\left(\frac{t_a(\omega)}{\theta_a(\omega)}\right) \cdot \sigma^*(a)
    \end{equation*}
\end{itemize}

An essential finding by \cite{ECTA12609} asserts that under mild conditions, such as the one outlined in \Cref{ass:discrete sets}, a Berk-Nash equilibrium is guaranteed to exist.

\begin{assumption}\label{ass:discrete sets}
    The sets of actions $\actions$, outcomes $\Omega$, and potential beliefs $\Theta$ are all finite. Furthermore, for each belief $\theta\in \Theta$ and each action $a\in \actions$, it holds that $\supp(\theta_a)=\supp(T_a)$.
\end{assumption}

The assumptions as stated in \Cref{ass:discrete sets} serve as a practical foundation for our analysis. The finiteness of the sets $\actions$, $\Omega$, and $\Theta$ simplifies the model and ensures the existence of solutions for the contract design problem. This set finiteness, though restrictive, represents an acceptable trade-off between mathematical tractability and real-world applicability. The equal support condition $\supp(\theta_a)=\supp(T_a)$ provides a common ground for comparing different belief-action pairs. This condition guarantees that there are no 'impossible' outcomes for any action according to the agent's belief, thereby aligning the belief space with the set of all possible outcomes. This alignment simplifies the analysis and allows for the examination of consistent, rational behavior on the part of the agent, given her available choices.


\begin{theorem}[Theorem~1 in \cite{ECTA12609}]
    For a mispecified contract design problem that meets the conditions of \Cref{ass:discrete sets}, a Berk-Nash equilibrium is certain to exist.\footnote{To reformulate a contract design an objective game in the sense of \cite{ECTA12609}, ...\rgn{fill in later.}}
\end{theorem}



\notshow{
\subsection{Objective Mechanism Design}

Mechanism design, often termed as 'reverse game theory', constitutes a significant field of study within Algorithmic Game Theory. It centers around formulating the rules or mechanisms of a game to attain certain desired outcomes, despite the non-observable actions of participants and their private information. The primary entity that designs the rules of the game is typically referred to as the 'designer' or 'principal', and the participants who play the game as per these rules are termed 'agents'.

A mechanism is formally characterized as a tuple $(S, g)$, where $S = S_1 \times S_2 \times \ldots \times S_n$ is the product space of the strategy sets for each agent, and $g: S \rightarrow \Theta$ is the outcome function. For each strategy profile $s \in S$ selected by the agents, the outcome function determines an outcome $g(s) \in \Theta$, where $\Theta$ represents the set of all potential outcomes.

Each agent has their individual utility function, denoted as $u_i: S \times \Theta \rightarrow \mathbb{R}$, which quantifies the agent's preference for each outcome given the selected strategies. Importantly, each agent typically has private information, and their utility function may also be privately known, which adds another layer of complexity in the design of the mechanism.

The aim of the designer in mechanism design is to create a game (mechanism) such that, in equilibrium, the resulting outcome optimizes a certain objective function. This could be, for instance, social welfare, fairness, revenue, etc., depending on the context of the game.

Mathematically, the designer’s objective could be represented as:

\begin{equation}
\max_{(S, g)} \mathbb{E}_{s \sim S} [f(g(s))],
\end{equation}

where $f: \Theta \rightarrow \mathbb{R}$ is the designer’s objective function. This function could represent the social welfare, revenue, fairness, or any other context-dependent objective of the game.

The primary challenge in mechanism design lies in crafting the rules of the game (i.e., the strategy spaces and the outcome function) such that, despite the agents' private information and non-observable actions, the equilibrium outcomes align with the designer's objectives. The field of mechanism design investigates various techniques and principles to tackle this challenge, such as incentive compatibility, revelation principles, and Vickrey-Clarke-Groves mechanisms.


\subsection{Berk Nash Equilibrium for Mispecified Agents}
The concept of the Berk-Nash equilibrium, originally developed within the realm of Game Theory, serves as a crucial analytical tool when considering strategic interactions amongst players. However, when the players, or agents, are misinformed or misperceive the game's parameters, a new concept arises known as the mis-specified Berk-Nash equilibrium.

In traditional game theory, a Berk-Nash equilibrium is a solution concept in which each player, given the strategies of other players, has no incentive to deviate unilaterally from their strategy. Yet, in many real-world scenarios, agents may misperceive the game structure or other players' strategies, leading to a situation where the agents' beliefs about the game do not align with the actual game.

The mis-specified Berk-Nash equilibrium takes into account these potential misperceptions and formulates a solution concept that reflects such situations. In a mis-specified Berk-Nash equilibrium, each agent, given their misperceptions about the game and the strategies of others, has no incentive to deviate from their strategy.

Formally, let $G$ denote the actual game and $G'$ denote the game as perceived by an agent. Let $s_i$ be the strategy chosen by player $i$, and let $s_{-i}$ be the strategies chosen by all other players. A strategy profile $s = (s_i, s_{-i})$ is a mis-specified Berk-Nash equilibrium if, for each player $i$,

\begin{equation}
\max_{s_i'} u_i(s_i', s_{-i}, G') \leq u_i(s_i, s_{-i}, G'),
\end{equation}

for all alternative strategies $s_i'$ that player $i$ could choose.

The mis-specified Berk-Nash equilibrium is a realistic and applicable concept, particularly when considering settings where agents' perceptions about the game may be incorrect due to lack of information, cognitive biases, or other factors. It helps model and analyze strategic interactions in these situations and provides insights into the possible outcomes and how misperceptions can impact the agents' strategies and the overall game outcomes.
}
